Assembly and measurements of the Electromagnetic Calorimeter components for "WASA at COSY" setup

This work describes the tests of the scintillator electromagnetic calorimeter of theWASA detector setup after transferring it from the CELSIUS storage ring at The Svedberg Laboratory(Uppsala, Sweden) to the Cooler Synchrotron COSY at the Institut fur Kernphysik (IKP) of Forschungszentrum Julich, Germany. The tests were performed using gammas of 4.4MeV energy from an AmBe source. The status of the CsI(Na) crystals was determined and the indication of gain factor for the energy calibration was extracted.

==> abstractDE.tex <==
\begin{otherlanguage}{german}
  \begin{abstract}
Diese Diplom Arbeit beschriebt die Teste des Elektromagnetisches Kalorimeter f\"ur WASA Detektor nach dem Transport von CELSIUM Akcelerator TSL(Uppsala, Sweden) nach Institut f\"ur Kernphysik (IKP) Forschungszentrum J\"ulich Deutschland. Das Kalorimeter wurde untersucht mit dem 4.4MeV Gamma Strahlen aus der AmBe Quelle. Der Zustand der CsI(Na) Kristalle wurde vorgestellt und das Konstant f\"ur Energie Kalibtation wurde gerechnet. 
  \end{abstract}
\end{otherlanguage}

